Correct-by-construction reach-avoid control of partially observable linear stochastic systems

We study feedback controller synthesis for reach-avoid control of discrete-time, linear time-invariant (LTI) systems with Gaussian process and measurement noise. The problem is to compute a controller such that, with at least some required probability, the system reaches a desired goal state in finite time while avoiding unsafe states. Due to stochasticity and nonconvexity, this problem does not admit exact algorithmic or closed-form solutions in general. Our key contribution is a correct-by-construction controller synthesis scheme based on a finite-state abstraction of a Gaussian belief over the unmeasured state, obtained using a Kalman filter. We formalize this abstraction as a Markov decision process (MDP). To be robust against numerical imprecision in approximating transition probabilities, we use MDPs with intervals of transition probabilities. By construction, any policy on the abstraction can be refined into a piecewise linear feedback controller for the LTI system. We prove that the closed-loop LTI system under this controller satisfies the reach-avoid problem with at least the required probability. The numerical experiments show that our method is able to solve reach-avoid problems for systems with up to 6D state spaces, and with control input constraints that cannot be handled by methods such as the rapidly-exploring random belief trees (RRBT).

==> Figures/2D/Table.tex <==
\begin{table}[t!]
\centering

\caption{Size of the abstract \gls{iMDP}, abstraction time, and satisfaction probability $p^\star_{\initState}$ as a function of the length of the transient phase $\bar{N}$ of the two-phase horizon.}
%
\begin{tabular}{lrrrr}
    \toprule
    \textbf{Transient phase length $\bar{N}$} &
    \textbf{1} & \textbf{3} & \textbf{5} & \textbf{7} \\
    \midrule
    Abstract \gls{iMDP} states $|S|$ & 
    $6\,053$ & $12\,103$ & $18\,153$ & $24\,203$ 
    \\
    Lower bound $p^\star_{\initState}$ ($\nu = 1$) &
    0.226 & 0.744 & 0.749 & 0.750
    \\
    Abstraction time ($\nu = 1$) [s] &
    59.6 & 80.1 & 106.9 & 131.3
    \\
    Lower bound $p^\star_{\initState}$ ($\nu = 0.1$) &
    0.516 & 0.975 & 0.983 & 0.983
    \\
    Abstraction time ($\nu = 0.1$) [s] &
    46.9 & 59.6 & 81.3 & 105.8
    \\
\bottomrule
\end{tabular}

\label{table:2D_drone}

\end{table}

==> Figures/3D/Table.tex <==
\begin{table}[t!]
\centering

\caption{Run times and \gls{iMDP} model sizes for the 3D \gls{UAV} benchmark, and the guaranteed satisfaction probability $\eta^\star \coloneqq p^\star_{\initState} - (1-\beta)(N+1)$ versus the empirical (simulated) satisfaction probability $\bar{p}_{\initState}$ as defined by \cref{eq:EmpiricalSatisfaction}.}
%
\begin{tabular}{llrrrr}
	\toprule
  \multicolumn{2}{c}{{\textbf{Noise strength}}} & \multicolumn{4}{c}{{\textbf{\gls{iMDP} model size}}} \\
  \cmidrule(lr){1-2} \cmidrule(lr){3-6}  
  Process & Measurement & States & Transitions & $\eta^\star$ & $\bar{p}_{\initState}$
  \\
\midrule
% Low  & Low all     & 2,455 & 30,843,102 & 0.992 & 1.000 \\
% Low  & High Z dir. & 2,441 & 33,664,546 & 0.986 & 1.000 \\
% Low  & High Y dir. & 2,435 & 33,560,234 & 0.986 & 1.000 \\
% High & Low all     & 3,140 & 83,529,922 & 0.729 & 0.980 \\
% High & High Z dir. & 3,115 & 82,832,745 & 0.621 & 0.994 \\
% High & High Y dir. & 3,123 & 82,740,497 & 0.645 & 0.988 \\
Low  & Low all     & 74\,847 & 30\,843\,102 & 0.992 & 1.000 \\
Low  & High Z dir. & 74\,847 & 33\,664\,546 & 0.986 & 1.000 \\
Low  & High Y dir. & 74\,847 & 33\,560\,234 & 0.986 & 1.000 \\
High & Low all     & 74\,847 & 83\,529\,922 & 0.729 & 0.980 \\
High & High Z dir. & 74\,847 & 82\,832\,745 & 0.621 & 0.994 \\
High & High Y dir. & 74\,847 & 82\,740\,497 & 0.645 & 0.988 \\
\bottomrule
\end{tabular}

\label{table:UAV_3D}

\end{table}
